Synchronous Faithfulness Monitoring for Trustworthy Retrieval-Augmented Generation

Retrieval-augmented language models (RALMs) have shown strong performance and wide applicability in knowledge-intensive tasks. However, there are significant trustworthiness concerns as RALMs are prone to generating unfaithful outputs, including baseless information or contradictions with the retrieved context. This paper proposes SynCheck, a lightweight monitor that leverages fine-grained decoding dynamics including sequence likelihood, uncertainty quantification, context influence, and semantic alignment to synchronously detect unfaithful sentences. By integrating efficiently measurable and complementary signals, SynCheck enables accurate and immediate feedback and intervention, achieving 0.85 AUROC in detecting faithfulness errors across six long-form retrieval-augmented generation tasks, improving prior best method by 4%. Leveraging SynCheck, we further introduce FOD, a faithfulness-oriented decoding algorithm guided by beam search for long-form retrieval-augmented generation. Empirical results demonstrate that FOD outperforms traditional strategies such as abstention, reranking, or contrastive decoding significantly in terms of faithfulness, achieving over 10% improvement across six datasets.

==> tables/backup/model_feature_and_alignscore.tex <==
\setlength{\tabcolsep}{3.5pt}
\begin{table}[]
  \centering
  % \resizebox{\columnwidth}{!}{%
  \resizebox{\linewidth}{!}{
  \begin{tabular}{l | c c c | c c c}
    \hline
    & \multicolumn{3}{c|}{\textbf{Llama-2-7B-chat}} & \multicolumn{3}{c}{\textbf{Mistral-7B-Instruct}} \\
    & QA & Summ & Data2txt & QA & Summ & Data2txt\\
    \hline
    Model features & 0.793$_6$ & 0.644$_6$ & 0.739$_2$ & 0.856$_3$ & 0.717$_2$ & 0.781$_1$ \\
    AlignScore & 0.772$_{\ }$ & 0.768$_{\ }$ & 0.679$_{\ }$ & 0.875$_{\ }$ & \textbf{0.829}$_{\ }$ & 0.731$_{\ }$ \\
    Combined & \textbf{0.833}$_3$ & \textbf{0.787}$_3$ & \textbf{0.785}$_2$ & \textbf{0.887}$_8$ & \textbf{0.829}$_0$ & \textbf{0.856}$_2$ \\
  \hline
  \end{tabular}
  }
  % \vspace{-2mm}
  \caption{\diwu{Combining model features and AlignScore; we can draw a bar plot instead.} \diwu{Model=MLP}}
  \label{tab:model_features_and_alignscore}
  % \vspace{-5mm}
  
\end{table}


==> tables/cross_task_detection.tex <==
\setlength{\tabcolsep}{3.5pt}
\begin{table}[]
  \centering
  % \resizebox{\columnwidth}{!}{%
  \resizebox{\linewidth}{!}{
  \begin{tabular}{l | c c c c }
    \hline
    Train vs. Test& FS & QA & Summ & Data2txt \\
    \hline
    FS & 0.764$_4$ & 0.817$_4$ & 0.754$_6$ & 0.755$_4$ \\
    QA & 0.763$_2$ & 0.833$_3$ & 0.733$_4$ & 0.748$_2$ \\
    Summ & 0.787$_3$ & 0.762$_3$ & 0.787$_3$ & 0.670$_1$ \\
    Data2txt & 0.770$_4$ & 0.803$_6$ & 0.735$_5$ & 0.785$_2$ \\
  \hline
  \end{tabular}
  }
  % \vspace{-2mm}
  \caption{\diwu{cross task detection with MLP on llama 2 7b chat; will convert this into a heatmap} \diwu{Note: average only counts cross-task detection and skips in-distribution detection} }
  \label{tab:cross_task_detection}
  % \vspace{-5mm}
  
\end{table}


==> tables/detection_ablations.tex <==
% \setlength{\tabcolsep}{3.5pt}
% \begin{table}[]
%   \centering
%   % \resizebox{\columnwidth}{!}{%
%   \resizebox{\linewidth}{!}{
%   \begin{tabular}{l | c c }
%     \hline
%     & Llama-2-7B-chat & Mistral-7B-Instruct \\
%     \hline
%     All Features & 0.731 & 0.785 \\
%     \ \ \ \ - Uncertainty & 0.681 (7\%$\downarrow$) & 0.731 (7\%$\downarrow$) \\
%     \ \ \ \ - Likelihood & 0.706 (3\%$\downarrow$) & 0.736 (6\%$\downarrow$) \\
%     \ \ \ \ - Context Influence & 0.678 (7\%$\downarrow$) & 0.705 (10\%$\downarrow$) \\
%     Uncertainty Only & 0.683 (7\%$\downarrow$) & 0.702 (11\%$\downarrow$) \\
%     Likelihood Only & 0.641 (12\%$\downarrow$) & 0.681 (13\%$\downarrow$) \\
%     Context Influence Only & 0.626 (14\%$\downarrow$) & 0.646 (18\%$\downarrow$) \\
%   \hline
%   \end{tabular}
%   }
%   % \vspace{-2mm}
%   \caption{\diwu{Ablation study with Logistic Regression}}
%   \label{tab:detection_ablation}
%   % \vspace{-5mm}
  
% \end{table}


\setlength{\tabcolsep}{3.5pt}
\begin{table}[]
  \centering
  % \resizebox{\columnwidth}{!}{%
  % \resizebox{\linewidth}{!}{
  \begin{tabular}{l | c c }
    \hline
    & Llama & Mistral \\
    \hline
    All Features & \textbf{0.831} & \textbf{0.867} \\
    \ \ \ \ - Uncertainty & 0.819 & 0.859  \\
    \ \ \ \ - Likelihood & 0.825 & 0.859  \\
    \ \ \ \ - Context Influence & 0.809 & 0.848 \\
    \ \ \ \ - Semantic Alignment & 0.751 & 0.798 \\
  \hline
  \end{tabular}
  % }
  % \vspace{-2mm}
  \caption{\diwu{Ablation study with MLP}}
  \label{tab:detection_ablation}
  % \vspace{-5mm}
  
\end{table}


==> tables/recontext_eval.tex <==
% \setlength{\tabcolsep}{3.5pt}
% \begin{table}[ht!]
%   \centering
%   % \resizebox{\columnwidth}{!}{%
%   % \resizebox{\linewidth}{!}{
%   \begin{tabular}{l | c c c | c }
%     \hline
%     & \multicolumn{3}{c|}{\textbf{Coherence}} & \multirow{2}{*}{\textbf{Adherence}}  \\
%     & $\uparrow$ & $=$ & $\downarrow$ & \\
%     \hline
%     QA & \\
%     Summ & \\
%     Data2txt & \\
%     Bio & \\
%     F-100 & \\
%     F-100-anti & \\
    
%   \hline
%   \end{tabular}
%   % }
%   % \vspace{-2mm}
%   \caption{\diwu{recontextualization evaluation}}
%   \label{tab:recontext_eval_results}
%   % \vspace{-5mm}
  
% \end{table}


\begin{figure*}[h!]
\small
\centering
\begin{tabular}{p{0.98\linewidth}}
    \hline
    \textbf{Input:} How to transfer water shares? \\
    \textbf{BT+LA+SEL:} \\
    Based on the provided passages, here's how water shares are transferred: 1. Passage 1 states that a fee of \$75.00 must be paid to process a Water Stock Certificate transfer. The passage also mentions that a new Water Stock Certificate will be issued to the new owner of record. 2. 3. Therefore, based on  the provided passages, the answer to the question is:  Transferring water shares involves paying a fee of \$75.00 to process the transfer, returning the Water Stock Certificate to the company, providing proof of ownership, and obtaining a new Water Stock Certificate in the new owner's name \\
    \textbf{BT+LA+SEL + Recontextualization:} \\
    Based on the provided passages, here's how water shares are transferred: First, a fee of \$75.00 must be paid to process the transfer. Then, a new Water Stock Certificate will be issued to the new owner of record. This process involves returning the Water Stock Certificate to the company, providing proof of ownership, and obtaining a new Water Stock Certificate in the new owner's name.  \\
    \hline     
    \textbf{Input:} What are some food that contain gluten? \\
    \textbf{BT+LA+SEL:} \\
    Based on the provided passages, here are some foods that contain gluten: 1. 2. \\
    \textbf{BT+LA+SEL + Recontextualization:}  \\
    Unable to answer.  \\
    \hline
    \textbf{Input:} What are some ways vinegar could be used for dogs? \\
    \textbf{BT+LA+SEL:} \\
    Based on the provided passages, here are some ways vinegar can be used for dogs: 1. Rejuvenates the coat and helps balance skin pH levels (Passage 1) 2. Improves skin and coat (Passage 2, point 1)3. Cleans the ears (Passage 2, points 2 and 3) 4. Repels fleas (Passage 2, point 3) 5. Fights fleas when bathed in an ACV-soap mixture (Passage 2, point 4) \\
    \textbf{BT+LA+SEL + Recontextualization:}  \\
    Based on the provided passages, vinegar can be used for dogs in several ways: 1. It rejuvenates the coat and helps balance skin pH levels, as mentioned in Passage 1. 2. It improves skin and coat, as mentioned in Passage 2. 3. It also cleans the ears, as mentioned in Passage 2 and 3. 4. It repels fleas, as mentioned in Passage 2, point 3) and fights fleas when bathed in an ACV-soap mixture, as mentioned in Passage 2.\\
    \hline
    \textbf{Input:} What are some exercises that tone the chest? \\
    \textbf{BT+LA+SEL:} \\
    Based on the provided passages, the following are exercises that tone the chest: 1. Modified tri-set for the chest (passage 2)  2. Pushups (passage 2)  3. \\
    \textbf{BT+LA+SEL + Recontextualization:}  \\
    Based on the provided passages, exercises that tone the chest include modified tri-set for the chest and pushups.
    \\
    \hline
\end{tabular}
\caption{Qualitative examples of the model fine-tuned for recontextualization. The outputs are collected from running BT+LA+SEL using Llama 2 7B Chat's outputs from the RAGTruth QA subset.}
\label{qualitative-study-recontextualization}
\end{figure*}

